Machine Learning for Experimental Design: Methods for Improved Blocking

Restricting randomization in the design of experiments (e.g., using blocking/stratification, pair-wise matching, or rerandomization) can improve the treatment-control balance on important covariates and therefore improve the estimation of the treatment effect, particularly for small- and medium-sized experiments. Existing guidance on how to identify these variables and implement the restrictions is incomplete and conflicting. We identify that differences are mainly due to the fact that what is important in the pre-treatment data may not translate to the post-treatment data. We highlight settings where there is sufficient data to provide clear guidance and outline improved methods to mostly automate the process using modern machine learning (ML) techniques. We show in simulations using real-world data, that these methods reduce both the mean squared error of the estimate (14%-34%) and the size of the standard error (6%-16%).

==> insets/tbl_coeff_controls2.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabularx}{\textwidth}{lCCCC}

\toprule
{Method}&{Mexico, n=100}&{Mexico, n=300}&{Sri Lanka, n=100}&{Sri Lanka, n=300} \tabularnewline
\midrule\addlinespace[1.5ex]
FPS: Random Forest&.0263533&.008179&.0363191&.0115406 \tabularnewline
Manual: BM Strata (48)&.0383383&.0107747&.0102974&.0082688 \tabularnewline
Manual: BM Strata (8)&.0340678&.0098922&.0385306&.0122537 \tabularnewline
No blocking&.0268958&.00846&.0342579&.0117433 \tabularnewline
VS: CART&.0285629&.0088137&.0370674&.0114494 \tabularnewline
VS: Lasso (1se) + CART&.0293496&.0094048&.0361346&.0111533 \tabularnewline
VS: Lasso + CART&.0291655&.0088588&.0356586&.0118031 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}


==> insets/tbl_se_controls.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabularx}{\textwidth}{lCCCC}

\toprule
{Method}&{Mexico, n=100}&{Mexico, n=300}&{Sri Lanka, n=100}&{Sri Lanka, n=300} \tabularnewline
\midrule\addlinespace[1.5ex]
FPS: Random Forest&1045.267&444.8927&1913.917&881.6229 \tabularnewline
Manual: BM Strata (48)&1257.313&503.5244&963.996&743.648 \tabularnewline
Manual: BM Strata (8)&1212.413&499.5222&1815.029&890.9506 \tabularnewline
No blocking&1060.695&450.1384&1860.998&884.7739 \tabularnewline
VS: CART&1076.312&430.2117&1927.623&889.7989 \tabularnewline
VS: Lasso (1se) + CART&1025.328&480.7565&1908.896&831.6432 \tabularnewline
VS: Lasso + CART&1034.414&438.904&1829.97&867.1517 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}

